An empirical evaluation of the usefulness of Tree Kernels for Commit-time Defect Detection in large software systems

Defect detection at commit check-in time prevents the introduction of defects into software systems. Current defect detection approaches rely on metric-based models which are not very accurate and whose results are not directly useful for developers. We propose a method to detect bug-inducing commits by comparing the incoming changes with all past commits in the project, considering both those that introduced defects and those that did not. Our method considers individual changes in the commit separately, at the method-level granularity. Doing so helps developers as they are informed of specific methods that need further attention instead of being told that the entire commit is problematic. Our approach represents source code as abstract syntax trees and uses tree kernels to estimate the similarity of the code with previous commits. We experiment with subtree kernels (STK), subset tree kernels (SSTK), or partial tree kernels (PTK). An incoming change is then classified using a K-NN classifier on the past changes. We evaluate our approach on the BigCloneBench benchmark and on the Technical Debt dataset, using the NiCad clone detector as the baseline. Our experiments with the BigCloneBench benchmark show that the tree kernel approach can detect clones with a comparable MAP to that of NiCad. Also, on defect detection with the Technical Debt dataset, tree kernels are least as effective as NiCad with MRR, F-score, and Accuracy of 0.87, 0.80, and 0.82 respectively.

==> MAP_and_Prec.tex <==

\begin{longtable}{lrrrrrr}
	\caption{5-statistic summary of the MAP for inter-project clone detection using PTK, STK, and SSTK tree kernels } 
	\label{table:map-intra}  \\
	\toprule
	 & \multicolumn{3}{c}{\textbf{Precision@K} }&
	 \multicolumn{3}{c}{\textbf{MAP}}\\
   	 \cmidrule(lr){2-4}  \cmidrule(lr){5-7}
	Statistic	& PTK & STK & SSTK & PTK  & STK  & SSTK \\
	\cmidrule(lr){1-1}	\cmidrule(lr){2-4} \cmidrule(lr){5-7}
		Min 	 &  0.0  &  0.0  &  0.0  &      &  & \\
		Q$_{1}$  & 50.0  & 30.0  & 40.0  &      &  &  \\
		Median   & 80.0  & 65.0  & 80.0  &      &  & \\
		Mean     & 72.5  & 0.25  & 64.1  &      &  &  \\
		Q$_{3}$  & 100.0 & 87.5  & 97.5  &      &  & \\
		Max      & 100.0 & 100.0 & 100.0 &      &  & \\
		\hline
\end{longtable}










==> Makefile <==
NAME=ICSME-draft
BIBTEX=bibtex
LATEX=latex
PDFLATEX=pdflatex
VIEWER=`cat ~/.viewer || which okular || which evince || which open`
LATEX_OPTS=-interaction=nonstopmode -halt-on-error

VPATH=.:Figures:figs:autofigs:figures



JPGS=$(patsubst %.jpg,%.eps,$(filter %.jpg,$(FIGS)))
GIFS=$(patsubst %.gif,%.eps,$(filter %.gif,$(FIGS)))
PNGS=$(patsubst %.png,%.eps,$(filter %.png,$(FIGS)))
SVGS=$(patsubst %.svg,%.eps,$(filter %.svg,$(FIGS)))
PDFS=$(patsubst %.pdf,%.eps,$(filter %.pdf,$(FIGS)))

EPSS=$(addsuffix .eps,$(basename $(FIGS)))


.PHONY: all clean default view push commit zip

default: view

all: $(NAME).pdf

$(NAME).pdf: $(NAME).tex *.bib $(EPSS)
	echo $(EPSS)
	$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex
	$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex
	$(BIBTEX) $(NAME)
	$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex
	$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex
	rm $(NAME).input.pdf $(NAME).good.pdf || true
	gs -q -dPDFA -dNOPAUSE -dBATCH -dSAFER \
	   -dPDFSETTINGS=/prepress \
	   -dAutoFilterColorImages=false \
	   -dAutoFilterGrayImages=false \
	   -dEmbedAllFonts=true \
	   -dAutoFilterMonoImages=false \
	   -dColorImageFilter=/FlateEncode \
	   -dGrayImageFilter=/FlateEncode \
	   -dMonoImageFilter=/FlateEncode \
	   -sDEVICE=pdfwrite \
	   -sOutputFile=$(NAME).good.pdf \
	   $(NAME).pdf
	mv $(NAME).pdf $(NAME).input.pdf
	cp $(NAME).good.pdf $(NAME).pdf

RTWO=response2
$(RTWO).pdf: *.cls $(RTWO).tex *.bib $(EPSS)
	echo $(EPSS)
	$(PDFLATEX) $(LATEX_OPTS) $(RTWO).tex
	$(PDFLATEX) $(LATEX_OPTS) $(RTWO).tex
	$(BIBTEX) $(RTWO)
	$(PDFLATEX) $(LATEX_OPTS) $(RTWO).tex
	$(PDFLATEX) $(LATEX_OPTS) $(RTWO).tex
	rm $(RTWO).input.pdf $(RTWO).good.pdf || true
	gs -q -dPDFA -dNOPAUSE -dBATCH -dSAFER \
	   -dPDFSETTINGS=/prepress \
	   -dAutoFilterColorImages=false \
	   -dAutoFilterGrayImages=false \
	   -dEmbedAllFonts=true \
	   -dAutoFilterMonoImages=false \
	   -dColorImageFilter=/FlateEncode \
	   -dGrayImageFilter=/FlateEncode \
	   -dMonoImageFilter=/FlateEncode \
	   -sDEVICE=pdfwrite \
	   -sOutputFile=$(RTWO).good.pdf \
	   $(RTWO).pdf
	mv $(RTWO).pdf $(RTWO).input.pdf
	cp $(RTWO).good.pdf $(RTWO).pdf


old$(NAME).pdf: *.cls $(NAME).tex *.bib $(EPSS)
	echo $(EPSS)
	$(LATEX) $(LATEX_OPTS) $(NAME).tex
	@if(grep "There were undefined references" $(NAME).log > /dev/null);\
	then \
		$(BIBTEX) $(NAME); \
		$(LATEX) $(LATEX_OPTS) $(NAME).tex; \
	fi
	@if(grep "Rerun" $(NAME).log > /dev/null);\
	then \
		$(LATEX) $(LATEX_OPTS) $(NAME).tex;\
	fi
	$(LATEX) $(LATEX_OPTS) $(NAME).tex
	dvips -j0 -Ppdf -Pbuiltin35 -G0 -z $(NAME).dvi

	gs -q -dPDFA \
	-dNOPAUSE -dBATCH -dSAFER -dPDFSETTINGS=/prepress \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dAutoFilterMonoImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dMonoImageFilter=/FlateEncode \
	-sDEVICE=pdfwrite -sOutputFile=$(NAME).pdf \
	-c .setpdfwrite \
	-f $(NAME).ps

clean:
	rm *.blg *.bbl *.log *.aux $(NAME).pdf $(NAME).dvi $(NAME).ps || echo Already Clean

view:	$(NAME).pdf
	$(VIEWER) $(NAME).pdf

$(SVGS) : %.eps : %.svg
	inkscape -b white -t -T --export-ignore-filters --export-eps=$@ $<

# Use PS pipeline for maximum compatibility with random latex packages

$(JPGS) : %.eps : %.jpg
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@
$(GIFS) : %.eps : %.gif
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@
$(PNGS) : %.eps : %.png
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@



%-crop.pdf: %.pdf
	pdfcrop $<

$(PDFS) : %.eps : %.pdf
	pdftops -eps $< $@

push:	commit
	git push

commit:
	git commit -av

zip : $(NAME).zip

$(NAME).zip : *.cls $(NAME).tex *.bib $(EPSS) Makefile
	zip $@ $^

x: $(NAME).pdf
	xournal $(NAME).pdf

titlepage.pdf: $(NAME).pdf
	#pdftk $(NAME).pdf cat 1 output titlepage.pdf
	pdflatex titlepage
	pdflatex titlepage
	#bibtex titlepage
	pdflatex titlepage
	pdflatex titlepage

#REV=5142dd5674dee074c9b90749cb129ade2cee1b86
REV=3fd915f39f40ed0f5d3e2ba6de44116eb61904a2
diff.pdf: *.cls $(NAME).tex *.bib $(EPSS)
	rm MLEnergyDraft-diff$(REV).tex || echo lol
	latexdiff-git -r $(REV) $(NAME).tex
	mv MLEnergyDraft-diff$(REV).tex diff.tex
	$(PDFLATEX) $(LATEX_OPTS) diff.tex
	$(PDFLATEX) $(LATEX_OPTS) diff.tex
	$(BIBTEX) diff
	$(PDFLATEX) $(LATEX_OPTS) diff.tex
	$(PDFLATEX) $(LATEX_OPTS) diff.tex

dist.zip: mkdist.sh
	bash mkdist.sh

commitview: $(NAME).pdf
	git log | head -n 1 | sed -e 's/^.* //' | xargs -i cp ICSME-draft.pdf {}.pdf
	git log | head -n 1 | sed -e 's/^.* //' | xargs -i xournal {}.pdf





==> RQ1_Table_MAP.tex <==

%%%%%%%%%%%%%%
\begin{table}
	\centering
	\caption{Mean Average Precision (MAP) per BigCloneBench functionality calculated using Subtree kernel (STK), Subset tree kernel (SSTK), and Partial tree kernel (PTK)}
	\label{table:ptk_map}
\begin{tabular}{l|r|r|r|r}
	\toprule
	\textbf{Description} & \textbf{Funct.}  & \textbf{STK} & \textbf{PTK} & \textbf{SSTK}\\ 
	\cmidrule(lr){1-1}
	\cmidrule(lr){2-2}
	\cmidrule(lr){3-3}
	\cmidrule(lr){4-4}	
	\cmidrule(lr){5-5}
	Download from Web &   2 & 0.11 & 0.13 & 0.12 \\ 
	Secure hash &   3 & 0.25 & 0.29 & 0.28 \\ 
	Unzip &   5 & 0.38 & 0.38 & 0.38 \\ 
	Connect to the FTP server/Login &   6 & 0.62 & 0.64 & 0.62 \\ 
	Sorts an array &   7 & 0.20 & 0.30 & 0.23 \\ 
	Setup SGV  &   8 & 0.15 & 0.14 & 0.16 \\ 
	Setup SGV Event Handler(listener) &   9 & 0.12 & 0.13 & 0.13 \\ 
	DB update and rollback &  10 & 0.58 & 0.59 & 0.59 \\ 
	Initialize java project &  11 & 0.93 & 0.93 & 0.93 \\ 
	Get Prime Factors &  12 & 0.34 & 0.44 & 0.41 \\ 
	Shuffle array in place &  13 & 0.24 & 0.31 & 0.28 \\ 
	Binary search &  14 & 0.15 & 0.23 & 0.18 \\ 
	Create font &  15 & 0.64 & 0.71 & 0.65 \\ 
	Create Encryption Key Files &  17 & 0.02 & 0.03 & 0.02 \\ 
	Play sound &  18 & 0.36 & 0.40 & 0.38 \\ 
	Take Screenshot to File &  19 & 0.26 & 0.30 & 0.27 \\ 
	Fibonacci &  20 & 0.99 & 0.99 & 0.99 \\ 
	XMPP send message &  21 & 0.40 & 0.43 & 0.45 \\ 
	Encrypt To File &  22 & 0.18 & 0.21 & 0.19 \\ 
	Resize Array &  23 & 0.79 & 0.85 & 0.80 \\ 
	Open URL in System Browser &  24 & 0.76 & 0.78 & 0.76 \\ 
	Open file in Desktop &  25 & 0.23 & 0.25 & 0.24 \\ 
	GCD &  26 & 0.03 & 0.07 & 0.03 \\ 
	Call Method Using Reflection &  27 & 0.55 & 0.62 & 0.60 \\ 
	Parse XML to DOM &  28 & 0.52 & 0.58 & 0.56 \\ 
	Convert Date String Format &  29 & 0.24 & 0.25 & 0.24 \\ 
	Zip Files &  30 & 0.58 & 0.61 & 0.59 \\ 
	File Dialog &  31 & 0.94 & 0.94 & 0.93 \\ 
	Send E-Mail &  32 & 0.87 & 0.88 & 0.87 \\ 
	CRC32 File Checksum &  33 & 0.83 & 0.83 & 0.84 \\ 
	Execute External Process &  34 & 0.86 & 0.88 & 0.87 \\ 
	Instantiate Using Reflection  &  35 & 0.90 & 0.91 & 0.90 \\ 
	Connect to Database  &  36 & 0.92 & 0.91 & 0.91 \\ 
	Load File into Byte Array &  37 & 0.17 & 0.23 & 0.19 \\ 
	Get MAC Address String &  38 & 0.84 & 0.83 & 0.85 \\ 
	Delete Folder and Contents &  39 & 0.46 & 0.55 & 0.50 \\ 
	Parse CSV File &  40 & 0.68 & 0.73 & 0.70 \\ 
	Transpose Matrix &  41 & 0.83 & 0.87 & 0.84 \\ 
	Extract Matches Using Reg &  42 & 0.88 & 0.88 & 0.88 \\ 
	Copy Directory &  43 & 0.32 & 0.44 & 0.37 \\ 
	Test Palindrome &  44 & 0.95 & 0.95 & 0.95 \\ 
	Write PDF File &  45 & 0.55 & 0.58 & 0.58 \\ 
	\bottomrule
\end{tabular}
\end{table}


==> RQ1_Table_Precision.tex <==
\begin{table}
	\centering
	\hs{Use 0 to 1.0}
	\caption{Precision@10 per BigCloneBench functionality calculated using Subtree kernel (STK), Subset tree kernel (SSTK) and Partial tree kernel (PTK). Median percentage values are reported. }
	\label{table:precisionK}
	\begin{tabular}{l|r|r|r|r}
		\toprule
		\textbf{Description} & \textbf{ID} & \textbf{STK} & \textbf{PTK} & \textbf{SSTK} \\ 
		
		\cmidrule(lr){1-1}
		\cmidrule(lr){2-2}
		\cmidrule(lr){3-3}
		\cmidrule(lr){4-4}	
		\cmidrule(lr){5-5}
		
		Download from Web &   2 &  10 & 20 &  20 \\ 
		Secure hash &   3 &  30 & 60 &  50 \\ 
		Unzip &   5 &  60 & 60 &  60 \\ 
		Connect to the FTP server &   6 &  80 & 90 &  80 \\ 
		Sorts an array &   7 &  20 & 80 &  40 \\ 
		Setup SGV  &   8 &  50 & 35 &  50 \\ 
		Setup SGV Event Handler &   9 &  30 & 30 &  40 \\ 
		DB update and rollback &  10 &  80 & 80 &  80 \\ 
		Initialize java project &  11 & 100 & 100 & 100 \\ 
		Get Prime Factors &  12 &  60 & 80 &  80 \\ 
		Shuffle array in place &  13 &  40 & 60 &  50 \\ 
		Binary search &  14 &   0 & 50 &  20 \\ 
		Create font &  15 &  80 & 80 &  80 \\ 
		Create Encryption Key Files &  17 &  10 & 0 &  10 \\ 
		Play sound &  18 &  30 & 50 &  40 \\ 
		Take screenshot to file &  19 &  20 & 40 &  30 \\ 
		Fibonacci &  20 & 100 & 100 & 100 \\ 
		XMPP send message &  21 &  50 & 60 &  70 \\ 
		Encrypt to file &  22 &  30 & 40 &  40 \\ 
		Resize array &  23 &  80 & 100 &  80 \\ 
		Open URL in system browser &  24 &  80 & 90 &  90 \\ 
		Open file in desktop &  25 &  40 & 40 &  40 \\ 
		GCD &  26 &   0 & 30 &   0 \\ 
		Call Method using Reflection &  27 &  70 & 100 & 100 \\ 
		Parse XML to DOM &  28 &  40 & 90 &  80 \\ 
		Convert Date String Format &  29 &  20 & 30 &  20 \\ 
		Zip Files &  30 &  80 & 90 &   0 \\ 
		File Dialog &  31 & 100 & 100 & 100 \\ 
		Send E-Mail &  32 & 100 & 100 & 100 \\ 
		CRC32 File Checksum &  33 &  90 & 90 &  90 \\ 
		Execute External Process &  34 & 100 & 100 & 100 \\ 
		Instantiate using Reflection  &  35 & 100 & 100 & 100 \\ 
		Connect to Database  &  36 & 100 & 100 & 100 \\ 
		Load File into Byte Array &  37 &  10 & 40 &  10 \\ 
		Get MAC Address String &  38 & 100 & 90 & 100 \\ 
		Delete Folder and Contents &  39 &  30 & 80 &  50 \\ 
		Parse CSV File &  40 &  80 & 100 &  90 \\ 
		Transpose Matrix &  41 &  80 & 100 &  90 \\ 
		Extract matches using Regex &  42 & 100 & 100 & 100 \\ 
		Copy Directory &  43 &  30 & 80 &  30 \\ 
		Test Palindrome &  44 & 100 & 100 & 100 \\ 
		Write PDF file &  45 &  70 & 80 &  80 \\ 
	\bottomrule
	\end{tabular}
\end{table}



==> RQ1_Table_combine.tex <==
\begin{table}[ht]
\centering
\caption{Percision@10 and Mean Average Precision (MAP) per BigCloneBench functionality calculated using Subtree kernel (STK), Subset tree kernel (SSTK), and Partial tree kernel (PTK)}
\label{table:ptk_map_prec}
\begin{tabular}{l|r|rrr|rrr}
  \toprule
  & Description & ID & STK & PTK & SSTK & STK\_MAP & PTK\_MAP & mAP\_SSTK \\ 
 	\cmidrule(lr){1-1}
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-5}
    \cmidrule(lr){6-8}	
  
	 Download from Web &   2 & 0.10 & 0.20 & 0.20 & 0.11 & 0.13 & 0.12 \\ 
	 Secure hash &   3 & 0.30 & 0.60 & 0.50 & 0.25 & 0.29 & 0.28 \\ 
	 Unzip &   5 & 0.60 & 0.60 & 0.60 & 0.38 & 0.38 & 0.38 \\ 
	 Connect to the FTP server/Login &   6 & 0.80 & 0.90 & 0.80 & 0.62 & 0.64 & 0.62 \\ 
	 Sorts an array &   7 & 0.20 & 0.80 & 0.40 & 0.20 & 0.30 & 0.23 \\ 
	 Setup SGV  &   8 & 0.50 & 0.35 & 0.50 & 0.15 & 0.14 & 0.16 \\ 
	 Setup SGV Event Handler(listener) &   9 & 0.30 & 0.30 & 0.40 & 0.12 & 0.13 & 0.13 \\ 
	 DB update and rollback &  10 & 0.80 & 0.80 & 0.80 & 0.58 & 0.59 & 0.59 \\ 
	 Initialize java project &  11 & 1.00 & 1.00 & 1.00 & 0.93 & 0.93 & 0.93 \\ 
	 Get Prime Factors &  12 & 0.60 & 0.80 & 0.80 & 0.34 & 0.44 & 0.41 \\ 
	 Shuffle array in place &  13 & 0.40 & 0.60 & 0.50 & 0.24 & 0.31 & 0.28 \\ 
	 Binary search &  14 & 0.00 & 0.50 & 0.20 & 0.15 & 0.23 & 0.18 \\ 
	 Create font &  15 & 0.80 & 0.80 & 0.80 & 0.64 & 0.71 & 0.65 \\ 
	 Create Encryption Key Files &  17 & 0.10 & 0.00 & 0.10 & 0.02 & 0.03 & 0.02 \\ 
	 Play sound &  18 & 0.30 & 0.50 & 0.40 & 0.36 & 0.40 & 0.38 \\ 
	 Take Screenshot to File &  19 & 0.20 & 0.40 & 0.30 & 0.26 & 0.30 & 0.27 \\ 
	 Fibonacci &  20 & 1.00 & 1.00 & 1.00 & 0.99 & 0.99 & 0.99 \\ 
	 XMPP send message &  21 & 0.50 & 0.60 & 0.70 & 0.40 & 0.43 & 0.45 \\ 
	 Encrypt To File &  22 & 0.30 & 0.40 & 0.40 & 0.18 & 0.21 & 0.19 \\ 
	 Resize Array &  23 & 0.80 & 1.00 & 0.80 & 0.79 & 0.85 & 0.80 \\ 
	 Open URL in System Browser &  24 & 0.80 & 0.90 & 0.90 & 0.76 & 0.78 & 0.76 \\ 
	 Open file in Desktop &  25 & 0.40 & 0.40 & 0.40 & 0.23 & 0.25 & 0.24 \\ 
	 GCD &  26 & 0.00 & 0.30 & 0.00 & 0.03 & 0.07 & 0.03 \\ 
	 Call Method Using Reflection &  27 & 0.70 & 1.00 & 1.00 & 0.55 & 0.62 & 0.60 \\ 
	 Parse XML to DOM &  28 & 0.40 & 0.90 & 0.80 & 0.52 & 0.58 & 0.56 \\ 
	 Convert Date String Format &  29 & 0.20 & 0.30 & 0.20 & 0.24 & 0.25 & 0.24 \\ 
	 Zip Files &  30 & 0.80 & 0.90 & 0.00 & 0.58 & 0.61 & 0.59 \\ 
	 File Dialog &  31 & 1.00 & 1.00 & 1.00 & 0.94 & 0.94 & 0.93 \\ 
	 Send E-Mail &  32 & 1.00 & 1.00 & 1.00 & 0.87 & 0.88 & 0.87 \\ 
	 CRC32 File Checksum &  33 & 0.90 & 0.90 & 0.90 & 0.83 & 0.83 & 0.84 \\ 
	 Execute External Process &  34 & 1.00 & 1.00 & 1.00 & 0.86 & 0.88 & 0.87 \\ 
	 Instantiate Using Reflection  &  35 & 1.00 & 1.00 & 1.00 & 0.90 & 0.91 & 0.90 \\ 
	 Connect to Database  &  36 & 1.00 & 1.00 & 1.00 & 0.92 & 0.91 & 0.91 \\ 
	 Load File into Byte Array &  37 & 0.10 & 0.40 & 0.10 & 0.17 & 0.23 & 0.19 \\ 
	 Get MAC Address String &  38 & 1.00 & 0.90 & 1.00 & 0.84 & 0.83 & 0.85 \\ 
	 Delete Folder and Contents &  39 & 0.30 & 0.80 & 0.50 & 0.46 & 0.55 & 0.50 \\ 
	 Parse CSV File &  40 & 0.80 & 1.00 & 0.90 & 0.68 & 0.73 & 0.70 \\ 
	 Transpose Matrix &  41 & 0.80 & 1.00 & 0.90 & 0.83 & 0.87 & 0.84 \\ 
	 Extract Matches Using Reg &  42 & 1.00 & 1.00 & 1.00 & 0.88 & 0.88 & 0.88 \\ 
	 Copy Directory &  43 & 0.30 & 0.80 & 0.30 & 0.32 & 0.44 & 0.37 \\ 
	 Test Palindrome &  44 & 1.00 & 1.00 & 1.00 & 0.95 & 0.95 & 0.95 \\ 
	 Write PDF File &  45 & 0.70 & 0.80 & 0.80 & 0.55 & 0.58 & 0.58 \\ 
  
  
  \bottomrule
\end{tabular}
\end{table}

==> RQ4_Table.tex <==

\begin{table}
	\caption{Defect Prediction performance of STK tree kernel on Technical Debt dataset. The performance is based on TopK accuracy (K=1 and K=5), Mean Reciprocal Rank (MRR), F-score, and Accuracy metric. }
	\label{table:TDD_kelp}  
	\begin{tabular}{l|rr|r|r|r}
	\toprule
	
	\textbf{Project} & \textbf{K=1} & \textbf{K=5} & \textbf{MRR} & \textbf{Accuracy} & \textbf{F-score} \\ 
	
	\cmidrule(lr){1-1}
	\cmidrule(lr){2-2}
	\cmidrule(lr){3-3}
	\cmidrule(lr){4-4}
	\cmidrule(lr){5-5}
	\cmidrule(lr){6-6}
	
	accumulo & 0.58 & 0.94 & 0.73 & 0.58 & 0.41 \\ 
	ambari 	 & 0.60 & 0.79 & 0.69 & 0.60 & 0.67 \\ 
	atlas    & 0.68 & 0.88 & 0.77 & 0.68 & 0.44 \\ 
	aurora & 0.94 & 0.98 & 0.96 & 0.94 & 0.90 \\ 
	batik    & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 \\ 
	beam     & 0.94 & 0.98 & 0.95 & 0.94 & 0.97 \\ 
	cocoon   & 0.93 & 0.96 & 0.94 & 0.93 & 0.96 \\ 
	commons-bcel & 0.64 & 0.94 & 0.77 & 0.64 & 0.78 \\ 
	commons-cli & 0.81 & 0.97 & 0.89 & 0.81 & 0.83 \\ 
	commons-codec & 0.75 & 0.89 & 0.82 & 0.75 & 0.81 \\ 
	commons-collections & 0.93 & 0.97 & 0.95 & 0.93 & 0.96 \\ 
	commons-dbcp & 0.71 & 0.95 & 0.82 & 0.71 & 0.64 \\ 
	commons-dbutils & 0.92 & 0.99 & 0.95 & 0.92 & 0.93 \\ 
	commons-digester & 0.74 & 0.80 & 0.77 & 0.74 & 0.81 \\ 
	commons-exec & 0.94 & 0.98 & 0.96 & 0.94 & 0.93 \\ 
	commons-fileupload & 0.92 & 0.93 & 0.93 & 0.92 & 0.95 \\ 
	commons-io & 0.63 & 0.88 & 0.72 & 0.63 & 0.69 \\ 
	commons-jelly & 0.87 & 0.96 & 0.91 & 0.87 & 0.92 \\ 
	commons-jexl & 0.66 & 0.88 & 0.76 & 0.66 & 0.73 \\ 
	commons-jxpath & 0.94 & 0.96 & 0.95 & 0.94 & 0.97 \\ 
	commons-net & 0.65 & 0.93 & 0.77 & 0.65 & 0.65 \\ 
	commons-validator & 0.93 & 0.96 & 0.94 & 0.93 & 0.95 \\ 
	commons-vfs & 0.80 & 0.96 & 0.87 & 0.80 & 0.88 \\ 
	felix & 0.82 & 0.91 & 0.86 & 0.82 & 0.77 \\ 
	httpcomponents-client & 0.89 & 0.93 & 0.91 & 0.89 & 0.94 \\ 
	httpcomponents-core & 0.94 & 0.97 & 0.95 & 0.94 & 0.97 \\ 
	mina-sshd & 0.94 & 0.97 & 0.96 & 0.94 & 0.35 \\ 
	santuario-java & 0.79 & 0.89 & 0.84 & 0.79 & 0.87 \\ 
	zookeeper & 0.85 & 0.95 & 0.89 & 0.85 & 0.49 \\ 
	\bottomrule
\end{tabular}
\end{table}


==> RQ5_Table.tex <==

\begin{table}
	\caption{Defect Prediction performance of our baseline NiCad clone detector on Technical Debt dataset. The performance is based on TopK accuracy (K=1 and K=5), Mean Reciprocal Rank (MRR), F-score, and Accuracy metric. }
	\label{table:TDD_nicad}
	\begin{tabular}{l|rr|r|r|r}
		\toprule
	
	
	%	\multicolumn{1}{c}{} &
	%	\multicolumn{2}{c}{}&
	%	\multicolumn{1}{c}{}&
	%	\multicolumn{1}{c}{}&
	%	\multicolumn{1}{c}{}\\
		
	%	\cmidrule(lr){2-3}
	%	\cmidrule(lr){4-4}
	%	\cmidrule(lr){5-5}
	%	\cmidrule(lr){6-6}
	
		
		\textbf{Project} & \textbf{K=1} & \textbf{K=5} & \textbf{MRR} & \textbf{Accuracy} & \textbf{F-score}\\ 
		\cmidrule(lr){1-1}
		\cmidrule(lr){2-2}
		\cmidrule(lr){3-3}
		\cmidrule(lr){4-4}
		\cmidrule(lr){5-5}
		\cmidrule(lr){6-6}
		
		accumulo & 0.62 & 0.76 & 0.68 & 0.62 & 0.38 \\ 
		ambari & 0.78 & 0.90 & 0.83 & 0.78 & 0.86 \\ 
		atlas & 0.50 & 0.61 & 0.55 & 0.74 & 0.56 \\ 
		attic-aurora & 0.82 & 0.88 & 0.85 & 0.82 & 0.83 \\ 
		batik & 0.98 & 0.99 & 0.99 & 0.98 & 0.99 \\ 
		beam & 0.97 & 0.97 & 0.97 & 0.97 & 0.99 \\ 
		cocoon & 0.97 & 0.97 & 0.97 & 0.97 & 0.98 \\ 
		commons-bcel & 0.83 & 0.85 & 0.84 & 0.83 & 0.90 \\ 
		commons-cli & 0.95 & 0.96 & 0.95 & 0.95 & 0.91 \\ 
		commons-codec & 0.82 & 0.90 & 0.86 & 0.82 & 0.85 \\ 
		commons-collections & 0.88 & 0.92 & 0.90 & 0.88 & 0.93 \\ 
		commons-dbcp & 0.90 & 0.95 & 0.92 & 0.90 & 0.73 \\ 
		commons-dbutils & 0.96 & 0.96 & 0.96 & 0.96 & 0.80 \\ 
		commons-digester & 0.73 & 0.87 & 0.79 & 0.73 & 0.73 \\ 
		commons-exec & 0.95 & 0.96 & 0.96 & 0.95 & 0.75 \\ 
		commons-fileupload & 0.88 & 0.89 & 0.89 & 0.88 & 0.91 \\ 
		commons-io & 0.62 & 0.91 & 0.74 & 0.62 & 0.65 \\ 
		commons-jelly & 0.72 & 0.76 & 0.74 & 0.72 & 0.82 \\ 
		commons-jexl & 0.70 & 0.91 & 0.79 & 0.70 & 0.67 \\ 
		commons-jxpath & 0.87 & 0.90 & 0.88 & 0.87 & 0.93 \\ 
		commons-net & 0.70 & 0.80 & 0.74 & 0.70 & 0.68 \\ 
		commons-validator & 0.94 & 0.95 & 0.94 & 0.94 & 0.95 \\ 
		commons-vfs & 0.68 & 0.78 & 0.72 & 0.68 & 0.76 \\ 
		felix & 0.96 & 0.97 & 0.96 & 0.96 & 0.96 \\ 
		httpcomponents-client & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\ 
		httpcomponents-core & 0.94 & 0.96 & 0.95 & 0.94 & 0.97 \\ 
		mina-sshd & 0.97 & 0.99 & 0.98 & 0.97 & 0.38 \\ 
		santuario-java & 0.78 & 0.90 & 0.84 & 0.78 & 0.85 \\ 
		zookeeper & 0.73 & 0.85 & 0.79 & 0.73 & 0.20 \\ 
		\bottomrule
	\end{tabular}
\end{table}


